Dynamic Sequential Graph Learning for Click-Through Rate Prediction

Click-through rate prediction plays an important role in the field of recommender system and many other applications. Existing methods mainly extract user interests from user historical behaviors. However, behavioral sequences only contain users' directly interacted items, which are limited by the system's exposure, thus they are often not rich enough to reflect all the potential interests. In this paper, we propose a novel method, named Dynamic Sequential Graph Learning (DSGL), to enhance users or items' representations by utilizing collaborative information from the local sub-graphs associated with users or items. Specifically, we design the Dynamic Sequential Graph (DSG), i.e., a lightweight ego subgraph with timestamps induced from historical interactions. At every scoring moment, we construct DSGs for the target user and the candidate item respectively. Based on the DSGs, we perform graph convolutional operations iteratively in a bottom-up manner to obtain the final representations of the target user and the candidate item. As for the graph convolution, we design a Time-aware Sequential Encoding Layer that leverages the interaction time information as well as temporal dependencies to learn evolutionary user and item dynamics. Besides, we propose a Target-Preference Dual Attention Layer, composed of a preference-aware attention module and a target-aware attention module, to automatically search for parts of behaviors that are relevant to the target and alleviate the noise from unreliable neighbors. Results on real-world CTR prediction benchmarks demonstrate the improvements brought by DSGL.

==> 3_DSG.tex <==
Given a list of historical user-item interaction tuples $\gE=\left\{\left(u, i,t\right)\right\}$ observed in a time window, each of which represents the user $u\in\gU$ interacts with an item $i\in\gI$ associated with an timestamp $t\in\sR^{+}$, for each user-item pair to be scored, the corresponding Dynamic Sequential Graph is constructed in a recursive way, and the process is as follows:
\begin{itemize}[leftmargin=*]
    \item For a user $u\in\gU$ (or an item $i\in\gI$) at time $t$, we define the $1$-depth dynamic sequential subgraph of user $u$ (or item $i$) at time $t$ as a set of interactions of user $u$ (or item $i$) before time $t$ in chronological order, denoted by $\gG_{u,t}^{(1)}=\{(u,i,\tau)|\tau<t,(u,i,\tau)\in\gE\}$ (or $\gG_{i,t}^{(1)}=\{(u,i,\tau)|\tau<t,(u,i,\tau)\in\gE\}$). In practice, we will take the last $m$ interactions before time $t$, where $m$ is a hyperparameter. 
    \item Given the $k$-depth dynamic sequential subgraphs $\gG_{i,t}^{(k)}$ for $i\in\gI$ (or $\gG_{u,t}^{(k)}$ for $u\in\gU$), we define the ($k$+1)-depth dynamic sequential subgraph of user $u$ (or item $i$) at time $t$ as a set of $k$-depth dynamic sequential subgraphs that user $u$ (or item $i$) interacts in chronological order with its $1$-depth dynamic sequential subgraphs, $\gG_{u,t}^{(k+1)}=\{\gG_{i,\tau}^{(k)}|\tau<t,(u,i,\tau)\in\gE\}\cup\gG_{u,t}^{(1)}$ (or $\gG_{i,t}^{(k+1)}=\{\gG_{u,\tau}^{(k)}|\tau<t,(u,i,\tau)\in\gE\}\cup\gG_{i,t}^{(1)}$).
\end{itemize}
In practice, we select the last $r$ interactions before time $t$ at each layer and control the number of layers to 2-4 layers to ensure DSG's lightweight from the perspective of efficiency.
The construction process of DSG is illustrated as Figure~\ref{fig:DSG}(b). 
% The $k$-order neighbor set for node $u$ (or node $i$) at the time $t$ is denoted by $\gN_{t}^k(u)$ (or $\gN_{t}^k(i)$). 
We define the historical behavior sequence of user $u$ (or item $i$) at time $t$ as a sequence of interacted items (or users) in chronological order, denoted by $\gS_{u,t}=\{(i,\tau)|\tau<t,(u,i,\tau)\in\gE\}$ (or $\gS_{i,t}=\{(u,\tau)|\tau<t,(u,i,\tau)\in\gE\}$).
\begin{figure}
    \centering
    \setlength\abovecaptionskip{2pt}
    \includegraphics[width=1.0\linewidth]{figure/DSG.eps}
    \caption{An example of an user's 3-depth dynamic sequential graph. DSG is constructed from bottom to top recursively.}
    \label{fig:DSG}
    \vspace{-0.3cm}
\end{figure}
\begin{table}[]
\centering
\setlength\abovecaptionskip{2pt}
\caption{Notations.}
\label{tab:not}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}ll@{}}
\toprule
Notation & Description \\ \midrule
    $\gE$   &   The user-item interaction set. \\ 
    $\gU,\gI$   &   The user and item set. \\ 
    $\gG_{u,t}^{(k)},\gG_{i,t}^{(k)}$    & The $k$-depth dynamic sequential subgraph at time $t$. \\  
    % $\gN^{k}_{t}(u),\gN^{k}_{t}(i)$   &   \makecell[l]{The $k$-order neighbor set of node $u$ and node $i$ at time $t$.} \\ 
    $\gS_{u,t},\gS_{i,t}$   &   The behavior sequence of user $u$ and item $i$ at time $t$. \\ 
    $b$ & The base of time bucket bounds.\\
     $\rvf_{user},\rvf_{item},\rvf_{time}$   &   The feature vectors of user $u$, item $i$ and time decay $t$. \\ 
     $\rve_{u,t},\rve_{i,t}$   &  \makecell[l]{The embedding vectors of user $u$ and item $i$ at time $t$ \\ after the embedding layer.} \\
     $\rvh_{u,t},\rvh_{i,t}$   &   \makecell[l]{The hidden states of user $u$ and item $i$  at time $t$ \\ after the time-aware sequence encoding layer.} \\ 
     $\rvx_{u,t}^{(k)},\rvx_{i,t}^{(k)}$   &   \makecell[l]{The aggregated embedding vectors of user $u$ and item $i$ \\ at time $t$ of layer $k$.} \\ 
     $\hat{\rvx}_{u,t},\hat{\rvx}_{i,t}$   &   \makecell[l]{The final embedding vectors of user $u$ and item $i$ .} \\
    $\Theta$    & The parameters in the model $\gF()$. \\ 
    \bottomrule
\end{tabular}
}
\vspace{-0.4cm}
\end{table}
Table~\ref{tab:not} lists the main notations used in the paper.

